Insights From the NeurIPS 2021 NetHack Challenge

In this report, we summarize the takeaways from the first NeurIPS 2021 NetHack Challenge. Participants were tasked with developing a program or agent that can win (i.e., 'ascend' in) the popular dungeon-crawler game of NetHack by interacting with the NetHack Learning Environment (NLE), a scalable, procedurally generated, and challenging Gym environment for reinforcement learning (RL). The challenge showcased community-driven progress in AI with many diverse approaches significantly beating the previously best results on NetHack. Furthermore, it served as a direct comparison between neural (e.g., deep RL) and symbolic AI, as well as hybrid systems, demonstrating that on NetHack symbolic bots currently outperform deep RL by a large margin. Lastly, no agent got close to winning the game, illustrating NetHack's suitability as a long-term benchmark for AI research.

==> CHANGES <==
v1.28 (2020-09-21):

  * jmlr.cls:

   Bug fixes: 

    - fixed twoside option (which should be the default)

    - \thanks now uses mpfootnote instead of footnote counter
      with matching \footnotemark and \footnotetext optional
      arguments.

v1.27 (2020-03-26):

  * jmlrutils.sty:

    Bug fix: subfigure and subtable references were producing
    extraneous text (added check for LaTeX kernel version)

v1.26 (2020-01-31):

  * jmlr.cls:

    - removed \vbox from \@jmlrmaketitle to allow for extremely long
      author/affiliation list. Added \ignorespaces before \@author
      to allow for spacing the contents in the code for clarity
      at the start of a long author list.

v1.25 (2020-01-17):

  * jmlr.cls: 

    - Added check for graphics.sty 2019/07/01 (which now detokenizes
      filename)

  * jmlrutils.sty:

    - Added \proofname

v1.24 (2017-08-01):

  * moved non-class related code into new package jmlrutils.sty

  * fixed bug in \includeteximage

v1.23 (2017-03-09):

  * added pmlr class option

v1.22 (2015-04-11):

  * added oneside and twoside class options

v1.21 (2015-02-24):

  * jmlr.cls

    - added check for jmlr2e and pseudocode

    - fixed bug in \thanks to fix footnote marker issue if there's
      more than one \thanks

  * jmlrbook.cls

    - added \nopagebreak after \@editorialteam

v1.20 (2014-10-15):

  * jmlrbook.cls

    - added \jmlrprefaceheader, \jmlrlocation

v1.19 (2014-09-29):

  * jmlrbook.cls

    - changed \chapter* to \chapter in preface environment

v1.18 (2013-10-17):

  * jmlrbook.cls

    - patched to work with auxhook

    - added draft and final options

    - add \booklinebreak

  * jmlr.cls

    - Added calc and etoolbox as required packages

    - Added draft and final options and removed \ds@draft

    - Added starred version of \newtheorem

    - Added \theorembodyfont, \theoremheaderfont, \theorempostheader
      and \theoremsep

v1.17 (2012-05-30):

  * jmlr.cls

    - added \titletag

    - added warnings if obsolete font commands (such as \bf) used

  * jmlrbook.cls

    - added 'articlet' page style

    - \importarticle sets title page style to articlet

    - \importpaper disables \jmlryear, \jmlrworkshop, \jmlrvolume
      and \jmlrissue

    - html title page uses jmlrvolume instead of volume

    - added optional argument to \logo

v1.16 (2012-05-15):

  * jmlr.cls

    - added \@post@hyperref hook

  * jmlrbook.cls

    - added code to deal with \c@lenddoca clash

v1.15 (2012-05-12):

  * jmlrbook.cls

    - added 'algocf' and 'definition' counters to reset list in
      \zeroextracounters

    - added \theHalgocf

    - removed dependence on \ps@headings in \ps@jmlrbook

    - added \markleft

v1.14 (2012-04-24):

  * jmlrbook.cls

    - modified \jmlrwritepdfinfo to write book author and title
      information to aux file
    - fixed bug in fetching time zone information

v1.13 (2012-02-25):

  * jmlrbook.cls

    - added pdfxa option
    - added \jmlrwritepdfinfo
    - changed preface environment to use \chapter* instead of \chapter

  * jmlr.cls

    - added \@pre@hyperref hook

v1.12 (2012-01-05):

  * jmlr.cls

    - removed prehyperref package option.

    - renamed \jmlr@prehyperref to \jmlrprehyperref

    - added tabularx to list of problem packages.

    - provided default value of \@shortitle

    - added \titlebreak

    - added optional argument to \Name
      (\jmlrauthors now redefines \@jmlr@authors instead of
      \@jmlrauthors)

    - added chapter number to \theHsection to ensure unique
      hyperlinks in book

  * jmlrbook.cls

    - Moved loading setspace and fink before jmlr.cls loaded

    - changed \thechapter to \theHchapter in definition of
      \theHalgorithm etc

    - added \theHfootnote, \theHtable, \theHfigure

    - in \importpubpaper etc, changed \@shortitle to \@title in toc

  * makejmlrbook v0.31

    - footnotes in abstract files changed to in-line parentheses.

    - --batchtex option now also passes "-interaction=batchmode" to
      htlatex

    - added debugging option --noexecute

v1.11 (2011-03-24):

  * jmlr.cls

    - fixed typo: WC\&P -> W\&CP

    - added \jmlrabbrnamelist (used by makejmlrbook)

  * jmlrbook.cls

    - now requires fink package

    - added preface environment and \prefacename

    - added algorithm2e old commands (in case some authors are using
      an older version).

  * makejmlrbook (v0.3):

    - added changes made by Olivier Chapelle to add JMLR menu on the
      left side of the page and use description environment for each
      paper of the TOC.

    - added --extractpreface option

    - set hyperref draft mode for abstract only html pages.

    - abstract html source files now input original aux files to allow
      for citations.

v1.10 (2011-01-05):

  jmlr.cls

  * now loads xkeyval

  * now loads hyperref (instead of jmlrbook loading it)

  * added class option prehyperref={stuff to do before hyperref loaded}

  * added class option tablecaption=<position> (where <position> can
    either be top or bottom).

  * fixed 10pt, 11pt and 12pt class options, which weren't having
    any effect.

  * modified \thanks to ensure hyperlink works correctly.

  * added \mdseries to definition of \addr.

  * added \startpage (used by jmlrmakebook).

  * modified \artpart and \bookpart to correct bookmark level number

  jmlrbook.cls

  * code loading hyperref moved to jmlr.cls

  * added 10pt, 11pt and 12pt class options.

  * Removed redundant redefinition of \@bookpart

  makejmlrbook (v0.2):

  * Uses \startpage to set initial page number for stand-alone 
    articles.

  * Makes subdirectories in html directory for each article.

  * copies any image files generated by tex4ht into html directory.

  * added time stamp at the end of each of the generated html file.

v1.09 (2010-12-01):

  jmlr.cls

  * now loads article.cls instead of scrartcl.cls

  * Fixed sub-captions so that they don't exceed the width of the
    sub-figure/table to which they refer.

  * added \nametag, \reprint, \algocfconts, \theHsubfigure,
    \booktocpreamble, \@partapp.

  * Made \objectref robust

  jmlrbook.cls

  * Reset start and end document hook to avoid problems caused by
    defining duplicate commands.

  * Moved redefinition of \jmlrpremaketitlehook outside of import
    macros.

  * Moved \refstepcounter from \jmlrmaketitlehook to
    \jmlrpremaketitlehook

  * Added \jmlrimporthook

  * Added \label to \jmlrmaketitlehook

v1.08 (2010-07-27):

  * Fixed \thanks so that the footnote symbol is raised and isn't
    followed by a full stop.

v1.07 (2010-06-30):

  * Added check for two column

v1.06 (2010-06-17):

  jmlr.cls

  * Added tablecaptiontop and tablecaptionbottom class options

v1.05:

  jmlrbook.cls

  * Added \productioneditors

v1.04:

  * Added Perl script makejmlrbook

  jmlrbook.cls

  * Added patch to fix references in print mode

  * Added code to work with makejmlrbook

  jmlr.cls

  * Added code to work with makejmlrbook

v1.03:
  jmlrbook.cls

  * Added patch to combnat

  jmlr.cls

  * Added \editors, \editorname and \editorsname

v1.02:
  jmlrbook.cls:

  * Added \issue

  jmlr.cls

  * Added \jmlrissue

v1.01 :

  jmlrbook.cls: 

  * added \importpaper

  * added \titlebody, \SetTitleElement and \IfTitleElement to 
    make it easier to customise the front page of the book.

  jmlr.cls:

  * fixed the last page anchor.

v1.0 : Initial release


==> INSTALL <==
INSTALLATION

*Installation is best performed using your TeX package manager.*
These are instructions for manual installation if for some reason a
package manager can't be used.

If you have downloaded the jmlr bundle using the TeX Directory
Structure (TDS), that is you have downloaded the archive
jmlr.tds.zip containing doc, tex and source directories, you need to
follow the "Installing from TDS" instructions below.

If you have downloaded the following files:

jmlr.dtx
jmlr.ins

You need to follow the "Installing from DTX and INS" instructions
below.

INSTALLING FROM TDS
===================

Files in tex and doc directories should go in the corresponding
TEXMF directories (for example, /usr/share/texmf-local/ or
C:\localtexmf\).

*Remember to refresh TeX's database*

Example (on UNIX like systems):

unzip jmlr.tds.zip -d ~/texmf/
texhash ~/texmf/

INSTALLING FROM DTX AND INS
===========================

Run LaTeX on jmlr.ins to generate jmlr.cls and jmlrbook.cls:

latex jmlr.ins

To create the documentation (jmlr.pdf):

pdflatex jmlr.dtx
makeindex -s gind.ist jmlr.idx
makeindex -s gglo.ist -o jmlr.gls jmlr.glo
pdflatex jmlr.dtx
pdflatex jmlr.dtx

If TEXMF denotes the base directory of your local TeX installation (e.g.
/usr/share/texmf-local/ or C:\localtexmf\) then create the following
directories (if they don't already exist):

TEXMF/doc/latex/jmlr
TEXMF/tex/latex/jmlr

Move the documentation to TEXMF/doc/latex/jmlr/

Move jmlrutils.sty, jmlr.cls and jmlrbook.cls to TEXMF/tex/latex/jmlr/

*Remember to refresh TeX's database*




==> makejmlrbook <==
#!/usr/bin/env perl
# File          : makejmlrbook
# Author        : Nicola L C Talbot
# Date          : 22nd March 2010
# Last Modified : 21st September 2020
# Version       : 0.33
# Description   : Given the name of a document using the
#                 jmlrbook class file, this script runs
#                 pdflatex (and possibly bibtex) on the
#                 imported articles and the main document.
# http://www.dickimaw-books.com/
#
# This file is distributed as part of the jmlr LaTeX bundle.
#
# *****
# This script is now obsolete and will be removed in later
# distributions. Use MakeJmlrBookGUI instead:
# https://www.dickimaw-books.com/software/makejmlrbookgui
# *****
#
# Copyright (c) 2006-2020 Nicola L.C. Talbot
# This work may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.3
# of this license or any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.3 or later is part of all distributions of LaTeX
# version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Nicola Talbot.

use Getopt::Long;
use File::Basename;
use File::Copy;
use Cwd;
use strict;

my $version = "0.33 (2020-09-21)";

my $eol = "\n";
my $dd  = '/';

if ($^O eq 'MSWin32')
{
  $eol = "\r\n";
  $dd = "\\";
}

my $showversion      = 0;
my $showhelp         = 0;
my $quiet            = 0;
my $batchtex         = 0;
my $online           = 1;
my $print            = 1;
my $html             = 1;
my $latexapp         = 'pdflatex';
my $bibtexapp        = 'bibtex';
my $latexopts        = '';
my $bibtexopts       = '';
my $format           = 'pdf';
my $logourl          = '';
my $extractpreface   = 0; # v0.3 added
# execute system calls (--noexecute will just list the system calls
# without executing them)
my $execute          = 1; # v0.31 added

my $appname = basename($0);

warn <<__END_OBSOLETE_WARN;
Warning: $appname is now obsolete and will be removed in later
distributions. Use MakeJmlrBookGUI instead:
https://www.dickimaw-books.com/software/makejmlrbookgui

__END_OBSOLETE_WARN

unless(&GetOptions(
   "online!"          => \$online,
   "print!"           => \$print,
   "html!"            => \$html,
   "extractpreface!"  => \$extractpreface,
   "logourl=s"        => \$logourl,
   "format=s"         => \$format,
   "latexapp=s"       => \$latexapp,
   "bibtexapp=s"      => \$bibtexapp,
   "latexopts=s"      => \$latexopts,
   "bibtexopts=s"     => \$bibtexopts,
   "quieter!"         => \$quiet,
   "batchtex!"        => \$batchtex,
   "execute!"         => \$execute,
   "version"          => \$showversion,
   "help"             => \$showhelp))
{
   die "Use --help for help\n";
}

if ($showhelp)
{
  die "$appname version $version Copyright (c) 2010 Nicola L C Talbot\n",
    "Distributed under the LaTeX Project Public License.\n\n",
    "Syntax: $appname [options] <filename>\n\n",
    "<filename> should be the name of the master document for a LaTeX \n",
    "file that uses the jmlrbook class. The .tex extension may be\n",
    "omitted.\n\n",
    "Basic options:\n",
    "--online\t\tGenerate the color on-line version (default)\n",
    "--noonline\t\tDon't generate the color on-line version\n",
    "--print\t\t\tGenerate the grayscale print version (default)\n",
    "--noprint\t\tDon't generate the grayscale print version\n",
    "--html\t\t\tGenerate the HTML version (default)\n",
    "--nohtml\t\tDon't generate the HTML version\n",
    "--extractpreface\tParse document for preface environment\n",
    "--noextractpreface\tDon't parse document for preface environment\n",
    "--logourl <url>\tMake the logo on the HTML index page link to <url>\n",
    "--batchtex\t\tRun TeX in batch mode\n",
    "--nobatchtex\t\tDon't run TeX in batch mode\n",
    "--quieter\t\tReduce messages to stdout and run TeX in batch mode\n",
    "--noquieter\t\tDon't reduce messages to stdout\n",
    "--execute\t\tExecute system calls (default)\n",
    "--noexecute\t\tDon't execute system calls, just list the\n",
    "\t\t\tcommands.\n",
    "--version\t\tDisplay version number and exit\n",
    "--help\t\t\tDisplay help message and exit\n",
    "\nAdvanced options:\n",
    "--latexapp <name>\tApplication used to call LaTeX\n",
    "\t\t\t(Defaults to 'pdflatex')\n",
    "--format <string>\tOutput format (default: 'pdf')\n",
    "--bibtexapp <name>\tApplication used to call BibTeX\n",
    "\t\t\t(Defaults to 'bibtex')\n",
    "--latexopt <string>\tOptions to pass to LaTeX\n",
    "--bibtexopt <string>\tOptions to pass to BibTeX\n";
}

if ($showversion)
{
  die "$appname version $version copyright (c) 2010 Nicola L C Talbot\n",
    "Distributed under the LaTeX Project Public License.\n";
}

unless ($#ARGV == 0)
{
   die "$appname: missing filename\n",
       "use --help for help\n";
} 

if ($quiet or $batchtex)
{
   $latexopts = '-interaction=batchmode '.$latexopts;
}

if ($quiet)
{
   $bibtexopts = '-terse '.$bibtexopts;
}

my ($main_name, $main_path, $main_suffix) 
  = fileparse($ARGV[0], '\.(tex|ltx)');

$main_suffix = '.tex' unless $main_suffix;

my $org_dir = cwd();

&chdirordie($main_path);

my $mainaux = "$main_name.aux";

# If the aux file doesn't exist or the aux file is older than
# the main file, run latex

if (not -e $mainaux or (-M $mainaux > -M "$main_name$main_suffix"))
{
   &latex($main_name);
}

my $main_bibdata = 0;
my @imports = ();
my %pagerefs = ();
my $preface_data; # v0.3 new
my @preface_editors = ();

# Parse aux file

&parsemainaux($mainaux);

# Replace any instances of \articlepagesref

foreach my $import (@imports)
{
   my $label = $import->{'label'};

   my $pages = $pagerefs{$label}->{'start'}.'--'
             . $pagerefs{$label}->{'end'};

   $import->{'author'}=~s/\\articlepagesref\s*\{$label\}/$pages/;
}

if ($html)
{
   # If the html files need to be created, make the directory
   # html-src, if it doesn't already exist

   unless (-d 'html-src')
   {
      &mkdirordie('html-src');
   }

   unless (-d 'html')
   {
      &mkdirordie('html');
   }

   if ($extractpreface) # v0.3 new
   {
      # If the preface needs to be extract, make a directory for it if
      # it doesn't already exist

      my $prefdir = &fname("html-src", $preface_data->{'OutFile'});

      unless (-d $prefdir)
      {
         &mkdirordie($prefdir);
      }

      my $prefbase = &fname($prefdir, $preface_data->{'OutFile'});

      &createprefacefile($prefdir, $prefbase);

      # Create the cfg file

      &createjmlrcfg("html-src", $preface_data->{'OutFile'});

      &chdirordie($prefdir);

      &latex($preface_data->{'OutFile'});
      &htlatex($preface_data->{'OutFile'}, 'jmlr');

      &chdirordie($org_dir, $main_path);

      # Check the appropriate subdirectory is in html directory

      my $outname = &fname('html', $preface_data->{'OutFile'});

      unless (-d $outname)
      {
         &mkdirordie($outname);
      }

      # Copy pdf file

      &copyordie("$prefbase.$format",
                &fname($outname, "$preface_data->{OutFile}.$format"));

      # Copy html file

      &copyhtml($preface_data->{'OutFile'}, $preface_data->{'OutFile'});
   }
}

# Iterate through each imported article

foreach my $import (@imports)
{
   my $label = $import->{'label'};
   my $importbase = &fname($import->{'path'}, $import->{'name'});

   # Check the aux file of this article

   my $aux = "$importbase.aux";

   # The aux file should exist because running LaTeX on the
   # main file will create the aux file.

   my $bibdata = 0;

   if (open AUX, $aux)
   {
      &message("Reading '$aux'...\n");

      while (<AUX>)
      {
         if (/\\bibdata\b/)
         {
            $bibdata = 1;
         }
      }
  
      close AUX;
   }
   elsif (not $execute)
   {
      warn "Can't open '$aux' - skipping\n";
   }
   else
   {
      die "$appname: Can't open '$aux' $!\n";
   }

   # Do we need a bibtex run?

   if ($bibdata)
   {
      my $log = "$importbase.log";

      # If the log file doesn't exist, run LaTeX

      unless (-e $log)
      {
         &chdirordie($import->{'path'});

         &latex($import->{'name'});

         &chdirordie($org_dir, $main_path);
      }

      open LOGFD, $log or die "$appname: Can't open '$log' $!\n";

      &message("Reading '$log'...\n");

      my $runbibtex = 0;

      while (<LOGFD>)
      {
         if (/There were undefined citations\./)
         {
            # Run bibtex and latex
            $runbibtex = 1;

            last;
         }
      }

      close LOGFD;

      if ($runbibtex)
      {
         &chdirordie($import->{'path'});

         &bibtex($import->{'name'});
         &latex($import->{'name'});

         &chdirordie($org_dir, $main_path);
      }
   }

   if ($html)
   {
      # If html is required, we also need pdf versions of the
      # individual articles.

      # v0.2 run latex even if pdf file exists to ensure start page 
      # number is correct.

      &chdirordie($import->{'path'});

      &latexstartpage($import->{'name'}, $pagerefs{$label}->{'start'});

      &chdirordie($org_dir, $main_path);

      # Do we need a rerun?

      if (&needs_rerun($importbase))
      {
         &chdirordie($import->{'path'});

         &latexstartpage($import->{'name'}, $pagerefs{$label}->{'start'});

         &chdirordie($org_dir,$main_path);
      }

      my $importdir = $import->{'path'};

      if ($importdir = '.')
      {
         $importdir = $import->{'name'};
      }

      # Check the appropriate subdirectory is in html-src

      my $name = &fname('html-src', $importdir);

      unless (-d $name)
      {
         &mkdirordie($name);
      }

      my $text = '';

      # Read the LaTeX file and store everything up to
      # the end of the abstract

      my $tex = "$importbase.tex";

      my $absfile = &fname("html-src", $importdir,
                           $import->{'name'}.'.tex');

      if ($execute)
      {
         open TEX, $tex or die "$appname: Can't open '$tex': $!\n";

         while (<TEX>)
         {
            # This doesn't handle complicated cases, such as
            # the author using \abstract ... \endabstract
            # or commenting out the abstract with conditionals
            if (/^([^%]*)\\end\{abstract\}/)
            {
               $text .= $&;
               last;
            }

            $text .= $_;
         }

         close TEX;

         # Add the 'html' class option:
         unless ($text=~
          s/^([^%]*)\\documentclass\s*\[(.*)\]/$1\\documentclass[$2,html]/m)
         {
           $text=~s/^([^%]*)\\documentclass\s*/$1\\documentclass[html]/m;
         }

         my $aux = "$importbase.aux";

         $aux=~s/\\/\//g if ($dd eq '\\');

         my $prebegindoc = '\\hypersetup{draft}' . $eol
                         . '\\makeatletter' . $eol
                         . "\\input{../../$aux}" . $eol
                         . '\\makeatother'
                         . $eol;

         my $begindoc = '';

         # Set the authors
         if (defined($import->{'author'}))
         {
            my $author = $import->{'author'};

            $author=~s/^([^;]*);/\\textbf{\\emph{$1};}/;

            $begindoc .= "\\jmlrauthors{$author}";
         }

         # Add content div

         # v0.31 modified \footnote to set the footnote text as in-line
         # parenthesis.

         $text=~s/^([^%\n\r\f]*)\\begin\{document\}/
                 $prebegindoc$&$begindoc
                 \\HCode{<div id="content">}
                 \\renewcommand{\\footnote}[2][]{ (\#2)}%$eol
                 /mx;

         # Create file containing the abstract

         open ABSFD,">$absfile" 
           or die "$appname: Can't create '$absfile': $!\n";

         print ABSFD "\\batchmode", $eol if ($batchtex or $quiet);

         my $texpath = $import->{path};

         $texpath=~s/\\/\//g if ($dd eq '\\');

         print ABSFD
           "\\makeatletter",$eol,
           "\\def\\input\@path{{../../$texpath/}}$eol",
           "\\makeatother",$eol,
           $text, $eol, 
           "\\HCode{", &htmltimestamp, "}", $eol,
           "\\HCode{</div>}", $eol,
           &htmlmenu, # v0.3 added by Olivier Chapelle
           "\\end{document}",$eol;

         close ABSFD;
      }
      else
      {
         &messagecall("Skipping creation of '$absfile'\n");
      }

      # Create the cfg file

      &createjmlrcfg("html-src", $importdir);

      # Run htlatex

      # Change directory
      &chdirordie("html-src", $importdir);

      &htlatex($import->{'name'}, 'jmlr');

      # Go back to main directory

      &chdirordie($org_dir, $main_path);

      # Copy the html file to the html directory, but rename
      # the css file to jmlr.css

      &copyhtml($importdir, $import->{'name'});

      # Check the appropriate subdirectory is in html directory

      my $outname = &fname('html', $importdir);

      unless (-d $outname)
      {
         &mkdirordie($outname);
      }

      # Copy pdf file

      &copyordie("$importbase.$format",
                 &fname($outname, "$import->{name}.$format"));
   }
}

# do we need to run bibtex on the main document?

if ($main_bibdata)
{
   &bibtex($main_name);
}

if ($online)
{
   &latexonline($main_name);

   # do we need a rerun?

   if (&needs_rerun($main_name))
   {
      &message("Rerun required\n");
      &latexonline($main_name);

      # check again

      if (&needs_rerun($main_name))
      {
         &message("Rerun required\n");
         &latexonline($main_name);
      }
   }
}

if ($print)
{
   &latexprint($main_name);

   # do we need a rerun?

   if (&needs_rerun($main_name))
   {
      &message("Rerun required\n");
      &latexprint($main_name);

      # check again

     if (&needs_rerun($main_name))
     {
        &message("Rerun required\n");
        &latexprint($main_name);
     }
   }
}

if ($html and $execute)
{
   # Make the index file

   my $indexfile = &fname('html-src', "index");

   my $preamble = '';

   open OUTFD, ">$indexfile.tex" 
    or die "Can't open '$indexfile.tex': $!\n";

   open INFD, "$main_name.tex"
     or die "Can't open '$main_name.tex': $!\n";

   print OUTFD "\\batchmode", $eol if ($batchtex or $quiet);

   print OUTFD
        "\\makeatletter",$eol,
        "\\def\\input\@path{{../}}$eol",
        "\\makeatother",$eol,
        "\\def\\jmlrgrayscale{0}",$eol;

   while (<INFD>)
   {
      unless
        (s/^([^%]*)\\documentclass\s*\[([^\]]*)\]/
           $1\\documentclass[$2,html]/x)
      {
         s/^([^%]*)\\documentclass\s*/$&\[html\]/;
      }

      s/^([^%]*)\\begin\{document\}/
        \\hypersetup{draft}$eol$&\\HCode{<div id="content">}/x;

      if (/^([^%]*)\\maketitle/)
      {
         $preamble .= join('', $1, "\\maketitle", $eol);
         last;
      }

      $preamble .= $_;
   }

   close INFD;

   # Find the book logo
   if ($preamble
     =~/\\logo\s*(?:\[[^\]]*\])?\s*\{(%\s*\n)?\\includegraphics\s*(\[[^\]]*\])?\{([^}]*)\}\}/m)
   {
      my $texpath = $3;
      my $orgtexpath = $texpath;
      $texpath=~s/\//\\/g if ($dd eq "\\");

      my $ext = '';

      if (-e $texpath)
      {
         &copyordie($texpath, 'html');

         &copyordie($texpath, 'html-src');
      }
      elsif (-e "$texpath.png")
      {
         &copyordie("$texpath.png", 'html');

         &copyordie("$texpath.png", 'html-src');

         $ext = '.png';
      }
      elsif (-e "$texpath.jpg")
      {
         &copyordie("$texpath.jpg", 'html');
         &copyordie("$texpath.jpg", 'html-src');

         $ext = '.jpg';
      }
      elsif (-e "$texpath.gif")
      {
         &copyordie("$texpath.gif", 'html');

         &copyordie("$texpath.gif", 'html-src');

         $ext = '.gif';
      }

      my $img = basename($texpath);
      
      if ($logourl)
      {
         $preamble=~s/
                  \\includegraphics(\[[^\]]*\])?\{$orgtexpath\}/
                  \\href{$logourl}{\\includegraphics${1}{$img$ext}}/mgx;
      }
      else
      {
         $preamble=~s/
                  \\includegraphics(\[[^\]]*\])?\{$orgtexpath\}/
                  \\includegraphics${1}{$img$ext}/mgx;
      }
   }

   print OUTFD $preamble, $eol;

   # Parse TOC

   my $toc = "$main_name.toc";

   # Add link to preface if required

   if ($extractpreface)
   {
      print OUTFD
         "\\begin{description}\\item[\\normalfont \\prefacename]", $eol;

      print OUTFD "\\textbf{\\emph{\\jmlrabbrnamelist{{",
                  join('},{', @preface_editors),
                  "}}};} ",
                  '\\csname @jmlrabbrvproceedings\\endcsname\\space',
                  '\\csname @jmlrvolume\\endcsname:',
                  $preface_data->{'Start'};

      unless ($preface_data->{'Start'} eq $preface_data->{'End'})
      {
         print OUTFD '--', $preface_data->{'End'};
      }

      print OUTFD ', \\csname @jmlryear\\endcsname\\newline', $eol;

      my $name = $preface_data->{'OutFile'};

      print OUTFD "[\\HCode{<a href=\"$name.html\">html</a>}] ",
                  "[\\HCode{<a href=\"$name/$name.pdf\">pdf</a>}]",
                  $eol;

      print OUTFD "\\end{description}$eol";
   }

   open TOC, $toc or die "Can't open '$toc': $!\n";

   my $idx = 0;

   while (<TOC>)
   {
      if (/^\\tocpart\s*\{(.*)\}\s*$/)
      {
         print OUTFD "\\begin{center}\\bfseries $1\\end{center}$eol";
      }
      elsif (/\\contentsline\s*\{papertitle\}\{(.*)\}\{[^{}]*\}\{[^{}]*\}\s*$/)
      {
         # v0.3 Changed by Olivier Chapelle to use description
         # environment instead of paragraph break
         print OUTFD "\\begin{description}\\item[\\normalfont $1]$eol";
      }
      elsif (/\\contentsline\s*\{chapterauthor\}\{(.*)\}\{[^{}]*\}\{[^{}]*\}\s*$/)
      {
         my $details = $1;
         $details=~s/([^;]*);/\\textbf{\\emph{$1};}/;

         my $label = $imports[$idx]->{'label'};
         my $pages = $pagerefs{$label}->{'start'}.'--'
                   . $pagerefs{$label}->{'end'};

         $details=~s/\\articlepagesref\s*\{$label\}/$pages/;

         # v0.3 Changed by Olivier Chapelle to use newline instead of par
         print OUTFD "$details\\newline$eol";

         my $name = $imports[$idx]->{'name'};

         print OUTFD "[\\HCode{<a href=\"$name.html\">abs</a>}] ",
                     "[\\HCode{<a href=\"$name/$name.pdf\">pdf</a>}]",
                     $eol;

         # v0.3 Changed by Olivier Chapelle to end description
         print OUTFD "\\end{description}$eol";

         $idx++;
      }
   }

   close TOC;

   # version 0.2 added time stamp

   print OUTFD "\\HCode{", &htmltimestamp, "}$eol";

   print OUTFD &htmlmenu; # v0.3 Added by Olivier Chapelle

   print OUTFD "\\HCode{</div>}\\end{document}$eol";

   close OUTFD;

   # Go into html-src directory and run htlatex

   &chdirordie('html-src');

   &htlatex("index", 'xhtml');

   &chdirordie('..');

   # Copy to html directory

   my $inname = &fname('html-src', 'index.html');
   my $outname = &fname('html', 'index.html');

   open INFD, $inname or die "Can't open '$inname': $!\n";

   open OUTFD, ">$outname" or die "Can't open '$outname': $!\n";

   while (<INFD>)
   {
      s/href="index.css"/href="jmlr.css"/;

      print OUTFD;
   }

   close OUTFD;

   close INFD;

   # v0.2 new:
   # Copy any images generated by htlatex to html/

   my @imagefiles = glob(&fname('html-src', "index*.png"));

   foreach my $imagefile (@imagefiles)
   {
      copy($imagefile, 'html');
   }
}
elsif ($html)
{
   &messagecall("chdir 'html-src'\n");
   &htlatex("index", 'xhtml');
}

# Return to original directory
chdir $org_dir;

# Subroutines

sub message{ print @_ unless ($quiet) }

sub messagecall{ print @_ if (not $quiet or not $execute) }

sub systemcall{
  my $cmd = shift;

  &messagecall($cmd, "\n");

  my $code = 0;

  $code = system($cmd) if ($execute);

  $code;
}

sub latex{
   my $file = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts, "\"$file\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }
}

# v0.2 new
sub latexstartpage{
   my $file = shift;
   my $page = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts,
     "\"\\def\\startpage{$page}\\input{$file}\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }
}

sub copyordie{
   my ($org, $dest) = @_;

   &messagecall("copy '$org' to '$dest'\n");

   if ($execute)
   {
      copy($org, $dest) or die "Can't copy '$org' to '$dest': $!\n";
   }
}

sub latexonline{
   my $file = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts,
     "\"\\def\\jmlrgrayscale{0}\\input{$file}\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }

   &copyordie("$file.$format", "$file-online.$format");
}

sub latexprint{
   my $file = shift;

   my $code = &systemcall(join(' ', $latexapp, $latexopts,
     "\"\\def\\jmlrgrayscale{1}\\input{$file}\""));

   if ($code)
   {
      die "**LaTeX run failed with exit code $code.**\n",
          "Check '$file.log' for details\n";
   }

   &copyordie("$file.$format", "$file-print.$format");
}

sub bibtex{
   my $file = shift;

   my $code = &systemcall(
                 join(' ', $bibtexapp, $bibtexopts, "\"$file\""));

   if ($code)
   {
      die "**BibTeX run failed with exit code $code.**\n",
          "Check '$file.blg' for details\n";
   }
}

sub needs_rerun{
  my $file = shift;
  my $rerun = 0;

  unless ($execute)
  {
     &messagecall("Skipping rerun check for '$file'\n");
     return 0;
  }

  # Scan log file for rerun message

  my $log = "$file.log";

  # If there's no log file a run is needed
  open LOGFD, $log or return 1;

  while (<LOGFD>)
  {
     if (/Rerun to get cross-references right\./)
     {
        $rerun = 1;
        last;
     }
  }

  close LOGFD;

  return $rerun;
}

sub fname{ join($dd, @_) }

# v0.3 new
sub chdirordie{
  my $dirname = &fname(@_);

  &messagecall("chdir '$dirname'\n");

  unless (chdir $dirname)
  {
     if ($execute)
     {
        die "$appname: Can't change directory to $dirname: $!\n";
     }
     else
     {
        warn "(Can't change directory to '$dirname')\n";
     }
  }
}

# v0.31 new
sub mkdirordie{
  my $dirname = &fname(@_);

  &messagecall("mkdir '$dirname'\n");

  unless (mkdir $dirname)
  {
     if ($execute)
     {
        die "$appname: Can't create directory '$dirname': $!\n";
     }
     else
     {
        warn "(Can't create directory '$dirname')\n";
     }
  }
}

# v0.2 new
sub htmltimestamp{
   my $timestamp = localtime;

   return "<hr><center>Page last modified on $timestamp.</center>";
}

# v0.3 Added by Olivier Chapelle
sub htmlmenu{
  return '
\\HCode{<div id="fixed"><br>}
\\HCode{<a align="right" href="http://www.jmlr.org" target=_top><img align="right" class="jmlr" src="http://jmlr.csail.mit.edu/jmlr.jpg" border="0"></a>}
\\HCode{<p><br><br>}
\\HCode{<p align="right"> <A href="http://www.jmlr.org/"> Home Page </A>}
\\HCode{<p align="right"> <A href="/papers"> Papers </A>}
\\HCode{<p align="right"> <A href="/author-info.html"> Submissions </A>}
\\HCode{<p align="right"> <A href="/news.html"> News </A>}
\\HCode{<p align="right"> <A href="/scope.html"> Scope </A>}
\\HCode{<p align="right"> <A href="/editorial-board.html"> Editorial Board </A>}
\\HCode{<p align="right"> <A href="/announcements.html"> Announcements </A>}
\\HCode{<p align="right"> <A href="/proceedings"> Proceedings </A>}
\\HCode{<p align="right"> <A href="/mloss">Open Source Software</A>}
\\HCode{<p align="right"> <A href="/search-jmlr.html"> Search </A>}
\\HCode{<p align="right"> <A href="/manudb"> Login </A></p>}
\\HCode{<br><br>}
\\HCode{<p align="right"> <A href="http://jmlr.csail.mit.edu/jmlr.xml">}
\\HCode{<img src="http://jmlr.csail.mit.edu/RSS.gif" class="rss" alt="RSS Feed">}
\\HCode{</A>}
\\HCode{</div>}
'
}

# v0.3 new
sub htlatex{
   my ($filename, $cfg) = @_;

   # unicode-related options suggested by Olivier Chapelle

   # v0.31 added latex options in 5th parameter

   my $code = &systemcall(join(' ', 'htlatex',
                  "\"$filename\"",
                  "\"$cfg,uni-html4\"",
                  "\" -cunihtf -utf8\"",
                  '""',
                  "\" $latexopts\""
                 ));

   if ($code)
   {
      die "$appname: htlatex failed with exit code $code.\n";
   }
}

#v0.3 new
sub createjmlrcfg{
   my $cfg = &fname(@_, "jmlr.cfg");

   unless ($execute)
   {
      &messagecall("Skipping creation of '$cfg'\n");
      return;
   }

   open CFG, ">$cfg" or die "$appname: Can't create '$cfg': $!\n";

print CFG <<END_CFG;
\\Preamble{html}
\\begin{document}
\\Css{div.maketitle {text-align:left;}}
\\Css{h2.titleHead {text-align:left;}}
\\Css{. {font-family:verdana,helvetica,sans-serif}}
\\Css{a {text-decoration:none;color:\\#3030a0}}
\\Css{.cmbx-10x-x-109{ font-weight: bold;}}
\\Css{.cmbxti-10x-x-109{ font-weight: bold; font-style: italic;}}
\\Css{\\#fixed {position:absolute; top:0; left:0; width:8em;
height:100\\%;}}
\\Css{\\#content {margin-top:1em; margin-left:10em;
margin-right:0.5em;}}
\\Css{img.jmlr {width: 7em;}}
\\Css{img.rss {width: 2em;}}
\\EndPreamble
END_CFG

# v0.3 Last four \Css lines above added by Olivier Chapelle
   close CFG;
}

#v0.3 new
# copy html from html-src/$dir/ to html/ and rename css file
sub copyhtml{
   my ($dir, $name) = @_;

   my $infile = &fname("html-src", $dir, "$name.html");

   my $outfile = &fname("html", "$name.html");

   unless ($execute)
   {
      &messagecall("Copy '$infile' to '$outfile'\n");
      return;
   }

   open INFD, $infile or die "Can't open '$infile': $!\n";

   open OUTFD, ">$outfile" or die "Can't open '$outfile': $!\n";

   while (<INFD>)
   {
      s/href="$name\.css"/href="jmlr.css"/;

      print OUTFD;
   }

   close OUTFD;

   close INFD;

   # Copy css file

   &copyordie("html-src/$dir/$name.css", "html/jmlr.css");
}

sub parsemainaux{
   my $mainaux = shift;

   &message("Reading '$mainaux'...\n");

   unless (open AUX, "$mainaux")
   {
      if ($execute)
      {
         die "$appname: Can't open '$mainaux' $!\n";
      }
      else
      {
         warn "(Can't open '$mainaux' - skipping)\n";
         return;
      }
   }

   while (<AUX>)
   {
      if (/\\bibdata\b/)
      {
         $main_bibdata = 1;
      }
      elsif (/\\\@jmlr\@import\{(.*)\}\{(.*)\}\{(.*)\}/)
      {
         my $import = 
           {
             label => $1,
             path  => $2,
             name  => $3
           };

         $import->{'name'} =~s/\.(tex|ltx)\Z//;

         push @imports, $import;
      }
      elsif (/\\contentsline\s*\{chapterauthor\}\{(.*)\}\{\}\{\}}\s*$/
        and $#imports > -1)
      {
         $imports[$#imports]->{'author'} = $1;
      }
      elsif (/^\\newlabel\s*\{([^\}]*)jmlrstart\}\{\{([^\}]*)\}\{([^\}]*)\}/)
      {
         my $label = $1;
      
         $pagerefs{$label}->{'start'} = $3;
      }
      elsif (/^\\newlabel\s*\{([^\}]*)jmlrend\}\{\{([^\}]*)\}\{([^\}]*)\}/)
      {
         my $label = $1;

         $pagerefs{$label}->{'end'} = $3;
      }
      elsif ($extractpreface) # v0.3 new
      {
         if (/^\\\@prefacestart\{([^\}]*)\}\{(\d*)\}/)
         {
            $preface_data->{'Start'} = $1;
            $preface_data->{'StartArabic'} = $2;
         }
         elsif (/^\\\@prefaceend\{([^\}]*)\}/)
         {
            $preface_data->{'End'} = $1;
         }
         elsif (/^\\\@prefacefile\{([^\}]*)\}\{([^\}]*)\}/)
         {
            $preface_data->{'File'}    = $1;
            $preface_data->{'OutFile'} = $2;
         }
         elsif (/^\\\@prefaceeditor\{(.*)\}/)
         {
            my $name = $1;
            $name=~s/\\\\.*//;
            push @preface_editors, $name;
         }
      }
   }

   # if preface is to be extracted, has the require data been found?

   if ($extractpreface)
   {
      unless ($preface_data->{'File'})
      {
         warn "$appname: Can't find preface information in aux file.\n",
              "Have you used the preface environment?\n";

         $extractpreface = 0;
      }
   }

   close AUX;
}

sub createprefacefile{
   my ($prefdir, $prefbase) = @_;

   my $prefout = "$prefbase.tex";

   &messagecall("Create preface file '$prefout'\n");

   return unless ($execute);

   # Open preface output file

   open PREFOUT, ">$prefout"
      or die "$appname: Can't open '$prefout': $!\n";

   print PREFOUT "\\batchmode", $eol if ($batchtex or $quiet);
   print PREFOUT "\\makeatletter", $eol;
   print PREFOUT "\\def\\input\@path{{../../}}", $eol;
   print PREFOUT "\\makeatother", $eol;

   # Get the book's preamble

   my $filename = "$main_name$main_suffix";

   open BOOK, $filename
     or die "$appname: Can't open '$filename': $!\n";

   while (<BOOK>)
   {
      if (/\\documentclass/)
      {
         unless (s/^([^%]*)\\documentclass\s*\[(.*)\]/$1\\documentclass[$2,html]/m)
         {
           s/^([^%]*)\\documentclass\s*/$1\\documentclass[html]/m;
         }

         print PREFOUT;
      }
      elsif (/^\\begin{document}/)
      {
         if ($preface_data->{'Start'}=~/^[clxvi]+$/)
         {
            print PREFOUT "\\pagenumbering{roman}%", $eol;
         }
         elsif ($preface_data->{'Start'}=~/^[CLXVI]+$/)
         {
            print PREFOUT "\\pagenumbering{Roman}%", $eol;
         }

         print PREFOUT 
           "\\setcounter{page}{",
           $preface_data->{'StartArabic'},
           "}%", $eol;

         # \hypersetup{draft} is used to suppress links.
         # (Only a partial document so internal links may be
         # dead. Also prevents unwanted tag before the DOCTYPE
         # line in the HTML file.)

         print PREFOUT
               "\\hypersetup{draft}", $eol,
               '\\makeatletter',
               "\\\@openrightfalse\\input{../../$main_name.aux}",
               '\\makeatother', $eol;

         print PREFOUT
               "\\providecommand{\\HCode}[1]{}", $eol,
               "\\title{\\prefacename}", $eol,
               "\\begin{document}", $eol,
               "\\HCode{<div id=\"content\">}", $eol;

         last;
      }
      else
      {
         print PREFOUT;
      }
   }

   close BOOK;

   # Preface file name will have '/' as directory divider

   my $preffile = $preface_data->{'File'};

   if ($dd eq "\\")
   {
      $preffile=~s/\//\\/g;
   }

   open PREFIN, $preffile
     or die "$appname: Can't open '$preffile': $!\n";

   my $scanning  = 0;

   while (<PREFIN>)
   {
      # This is fairly primitive and works best when the begin
      # and end of the environment are on their own line.

      if (/\\begin\{preface\}/)
      {
         print PREFOUT;
         $scanning = 1;
      }
      elsif ($scanning)
      {
         print PREFOUT;

         last if /\\end\{preface\}/;
      }
   }

   close PREFIN;

   print PREFOUT
     "\\HCode{", &htmltimestamp, "}", $eol,
     "\\HCode{</div>}", $eol,
     &htmlmenu,
     "\\end{document}", $eol;

   close PREFOUT;

}

1;


==> sample-papers/images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}

